Multi-Tour Set Traveling Salesman Problem in Planning Power Transmission Line Inspection

This letter concerns optimal power transmission line inspection formulated as a proposed generalization of the traveling salesman problem for a multi-route one-depot scenario. The problem is formulated for an inspection vehicle with a limited travel budget. Therefore, the solution can be composed of multiple runs to provide full coverage of the given power lines. Besides, the solution indicates how many vehicles can perform the inspection in a single run. The optimal solution of the problem is solved by the proposed Integer Linear Programming (ILP) formulation, which is, however, very computationally demanding. Therefore, the computational requirements are addressed by the combinatorial metaheuristic. The employed greedy randomized adaptive search procedure is significantly less demanding while providing competitive solutions and scales better with the problem size than the ILP-based approach. The proposed formulation and algorithms are demonstrated in a real-world scenario to inspect power line segments at the electrical substation.

==> src/remove.tex <==
% Filename: remove.tex
% Date:     2020/10/15 17:19
% Author:   Jan Faigl

% - abstract.tex --------------------------------------------------------------
%Length constraints on individual routes are present, and cities to be visited are grouped in sets.
We present a formulation of integer linear programming to obtain optimal solution, and propose a metaheuristic greedy random adaptive search procedure to obtain solutions for large instances of this problem.

In the proposed formulation, we consider a limited travel budget of the inspection vehicle. 

% - introduction.tex ----------------------------------------------------------

%TheThe next step is performing those inspections autonomously, which is as of now an area of development. 
%We study part of an autonomous approach, which is the planning for time-optimal inspection of PTL infrastructure using an autonomous UAV.
%, where the goal is lowest total distance traveled by the salesman (ie. lowest total cost of traversed graph edges).The sequence of transmission line segments, and a general path, has to be determined before some flight trajectory is formed. 
, where the goal is lowest total distance traveled by the salesman (ie. lowest total cost of traversed graph edges).
This can be further generalized, so that the nodes are grouped in sets, where only one visit of city in a set is mandatory. 

Furthermore, we can considere multiple vehicles to visit the sets, or visiting 
Another generalization is to visit these sets using multiple salesmen at the same time, or using multiple tours of one salesman, starting and ending their respective tours in a single depot.

the segment and 
and it is proposed how to obtain solutions.
The salesman (UAV) is required to visit each segment of PTL, connecting PTL pylons, exactly once, and in arbitrary direction. The cost of travel to the segment and of the segment traversal itself is also relevant, 

problem, which can be solved to obtain a near optimal planning solution, and a greedy random search adaptive procedure (GRASP)~\cite{} is also proposed to solve it, since linear program is difficult to solve for combinatorically large instances.
%GRASP for fast solution
The targets of the inspection might change , and this paper describes a metaheuristic planner which is able to provide a fast, good-enough solution. 

% - related.tex ---------------------------------------------------------------

A general overview of multiple salesman problem solving procedures is provided by~\cite{bektas06omega}. 
The problem is also formulated as an ILP, proposed in \cite{miller60ilptsp}.
Our GRASP procedure is based on algorithm proposed in \cite{guemri16or}, which solves similar multi-product multi-vehicle inventory routing problem, which is a generalization of an inventory routing problem specified in \cite{bertazzi12jtl}. 
The procedure is fine-tuned with guidance of work discussing the specifics of tabu-search algorithms \cite{tsub98tabu}.

A combination of  heuristic 
Multiple-TSP scheme for UAV based 
, with a suitable heuristics and an integer programming formulation.

\cite{Piriyaniti2013} proposes a variant of variable neighborhood search of general asymmetric TSP. 
\cite{Ashraf2020} describes a hybrid algorithm based on ant colony optimization for TSP.
\cite{Yang2008} describes ant colony optimization for generalized set-TSP.
\cite{Salman2020} describes an algorithm for precedence-constrained set-TSP. 
In \cite{Yuan2020}, linear programming formulations and a heuristic is provided for set-TSP with time windows. 
Another hybrid algorithm based on Tabu Search is presented in \cite{Kucukoglu2019} for TSP with time windows, which considers agent recharging.
\cite{Bruni2020} describes a GRASP heuristic for multiple-TSP, with profits and uncertain travel times.
A water-flow alike algorithm for solving TSP is described in \cite{Othman2017}.

\disable{
Various recent approaches to either the MTSP or STSP problems exist and are mentioned here.
A combination of the meta-heuristic approach with the ant colony optimization (ACO) in a hybrid algorithm for the TSP is presented in~\cite{Ashraf2020}. Inspired by this, we also employ a hybrid approach when initializing the ILP solver using a solution obtained from our meta-heuristic solver.
ACO-based approach to the generalized set-TSP is described in~\cite{Yang2008}, and precedence-constrained set-TSP is addressed in~\cite{Salman2020}.
The set-TSP with time windows is addressed by heuristic and linear programming formulation in~\cite{Yuan2020}.
A variant of the TSP with time windows motivated by an electric vehicle with recharging has been addressed in~\cite{Kucukoglu2019}.
A GRASP heuristic for the MTSP with profits and uncertain travel times is described in~\cite{Bruni2020}.
}

localic, which can thus need to be considered in autonomous navigation.

The inspection planning can be formulated as the TSP~\cite{galceran13coverage}.
\textcolor{green}{TSP was previously used in inspection planning~\cite{tsp-in-ptl}, where inspection of pylon components is addressed using a Genetic Algorithm (GA). 
The same issue, along with PTL corridor inspection is explored in \cite{path-alg-uav}, where maximum flight distance limit is taken into account and both issues are formulated as a TSP and solved using a GA.
S
Similar issue, formulated as Two Layer Routing problem is explored in\cite{2lrouting}, where inspection of wiring is taken into account, but uses coordinated inspection by both ground vehicle and UAV.}


For a multi-route inspection, we may consider a variant of the Multiple Traveling Salesmen Problem (MTSP)~\cite{bektas06omega} that can be formulated using the ILP~\cite{miller60ilptsp}. This is, however, known to be very computationally demanding.

Alternatively, a less demanding heuristic GRASP has been employed in~\cite{guemri16or} for a problem similar to the PTL problem addressed in this paper. 

   %Standard TSP has in addition been solved using Particle Swarm \cite{tsp-particle} and Ant Colony \cite{tsp-ant} optimizations.

Various biologically inspired methods have been used for 

   ~\cite{hao08bio}, also called Generalized TSP in literature.
The problem was also formulated previously as an ILP~\cite{LAPORTE87stsp}. 

Regarding vision-based inspection, binocular depth imaging can be utilized for visual defect detection~\cite{mao19binocular} and~\cite{hui19overhead} reports on an imaging detail enhancement method in overhead visual inspection.
Robust visual detection and tracking of power-lines during inspection flight is evaluated in ~\cite{mendenez16vision}, and~\cite{zhou16tracking} reports on experimentally verified real-time automated tracking of power lines using a multi-rotor UAV.
While power lines do not significantly interfere with the global navigation satellite system (GNSS)~\cite{silva02gps}, the PTL magnetic field disrupts the magnetic compass on the UAV, affecting autonomous navigation.
Therefore, visual navigation using PTL pylons is a suitable solution, as described in~\cite{hui17navi}.



% - problem.tex ---------------------------------------------------------------
The goal is to traverse all segments of power-line, which lie between specified pylons, in shortest amount of time. 
Multiple tours are allowed, as long as they begin and end in the same specific depot. 
Multiple physical power-lines consisting of multiple connected segments can be included in planning at the same times. 
The direction, in which segment is traversed, is arbitrary. 
Therefore, visit of each segment is a visit of a vertex in some set, where every set should be visited exactly once. 
It is assumed that the problem being solved is practical one. Practicality in this case means that an UAV has limited flight time of several minutes ($\SI{20}{min}$ are assumed), and also has a limited flight speed, with which it can inspect power-line segments ($\SI{1}{m.s^{-1}}$). Flight speed while not inspecting a power-line is higher ($\SI{2}{m.s^{-1}}$). The problem size is then limited by real-world constrains.

Physical power-line pylons are referenced as capital letters of the alphabet ($A, B,\ldots, n_{pylon}$). 
The problem can be described as a weighted oriented graph search.
$V_{0}$ is a vertex representing starting depot, and $V_{1}$ is a vertex representing tour termination depot. 
They are separate vertices for the purpose of ILP formulation in Section~\ref{sec:ilp}, yet they have the same physical coordinates.
$V = \{2,\ldots,n_{vertex}\}$ are graph vertices, representing power-line segment visits in both directions (i.e. $AB, BA, BC\ldots$), where each pair of vertices referring to the same physical segment belongs to a set ($s_{A,B} = \{ AB, BA\}$). 
Each set $s_{i,j}$ has to be visited exactly once.
$S = \{0,\ldots,n_{set}\}$ are all formulated sets. 
Every power-line contributes $n-1$ segments and $2(n-1)$ vertices to the problem, where $n$ is number of pylons in the power-line.
$E = \{0,\ldots,n_{edge}\}$ are graph edges. 
For example, an edge $e_{(AB,CD)}$ represents route from pylon $B$, in which previous segment traversal from $A$ to $B$ terminated, to the beginning of the next segment $C$ and traversal of this segment from $C$ to $D$.
Cost of this edge $c(e)$ is the time spent on traveling to the target segment  added to time spent on traversing it.
$M = \{0,\ldots,n_{tour}\}$ are tours, all originating in vertex $V_{0}$ and terminating in vertex $V_{1}$. 
Cost of a tour $m$ is denoted as $c(m)$, and it is the sum of all graph edge costs $c(e), e \in m$ traversed by the tour. A tour contains series of graph edges/vertices it traverses/visits, the representations are equal.
Special case are edges connecting the depot to segments. While edges originating in $V_{0}$ have their cost assigned in the same way as other graph edges, the cost of an edge coming from some segment to the depot vertex is just the time of travel between them, since depot vertex does not represent edge traversal.

Definition of the goal to be minimized, which for one agent multi-tour scenario is the min-sum of all tour costs:
\begin{equation}
   \min \sum_{m\in M}c_m = \sum_{m\in M}\sum_{e_{i,j}\in m}c_{e_{i,j}},
\end{equation}
constrained to maximum tour cost (maximum flight time):
\begin{equation}
   \sum_{e_{i,j}\in m}c_{e_{i,j}} \leq T_\mathrm{max}, \forall m \in M.
\end{equation}
Had we chosen to use several UAVs at the same time, instead of one UAV making repeated tours, it would make sense to minimize maximum of all tour costs. This formulates a generalized set multiple-tours traveling salesman problem with budget constraint.

The problem domain can be described as a weighted oriented graph $G = (V,E)$ with a set of vertices $V$ that represents visits to power-line segments and a set of edges $E$ width the associated cost of travel between the segments.

Each vertex $v\in V$ physically represents a power-line segment between two pylons in a specific direction.
For an illustrative purpose, four example physical power-line pylons and segments between them can be referred to by capital letters of the alphabet, i.e., pylons $P_A, P_B, P_C, P_D$.


$V_{0}$ is a vertex representing starting depot, and $V_{1}$ is a vertex representing tour termination depot. 

A power-line segment can be visited in an arbitrary directions, e.g., $AB$ and $BA$ for the pylons $P_A$ and $P_B$, and thus the segment is represented by the set of vertices $s_{i,j}$ where each pair of pylons referres to the same physical segment, e.g., $s_{A,B} = \{ AB, BA\}$, and each set $s_{i,j}$ has to be visited exactly once.

They are separate vertices for the purpose of ILP formulation in Section~\ref{sec:ilp}, yet they have the same physical coordinates.
%   \caption{Representation of geometric path in the oriented graph. 
%   Travel from some segment end-point and traversal of next segment in specific direction is represented as a link in the oriented graph. }\label{fig:geometry}

For example, an edge $e_{AB,CD}$ represents route from pylon $B$, in which previous segment traversal from $A$ to $B$ terminated, to the beginning of the next segment $C$ and traversal of this segment from $C$ to $D$ as shown in~\ref{fig:geometry}.

Therefore, the vertices are partitioned into $n_{s}+2$ sets, 
, e.g., $AB$ and $BA$ for the pylons $P_A$ and $P_B$. and thus the segment is represented by the set of vertices $s_{i,j}$ where each pair of pylons referres to the same physical segment, e.g., $s_{A,B} = \{ AB, BA\}$, and each set $s_{i,j}$ has to be visited exactly once.

%$n_s$ 
%$n segments $ 
$V = \{2,\ldots,n_{vertex}\}$ are graph vertices, representing power-line segment visits in specific directions
$S = \{0,\ldots,n_{vertex}/2\}$ are all formulated sets. 
$E = \{0,\ldots,n_{edge}\}$ are graph edges. 
Edges can be referred to using integer indices of $V$, ie. $e_{AB,CD} = e_{1,3}$.
traveling to some target power-line segment from the end-point of previous segment added to time spent on traversing the target segment.

Cost of a tour $m$ is denoted as $c(m)$, and it is the sum of all graph edge costs $c(e), e \in m$ traversed by the tour. A tour contains series of graph edges/vertices it traverses/visits, the representations are equal.

%finish here
$M = \{0,\ldots,n_{tour}\}$ are tours, all originating in vertex $V_{0}$ and terminating in vertex $V_{1}$. 
Special case are edges connecting the depot to segments. While edges originating in $V_{0}$ have their cost assigned in the same way as other graph edges, the cost of an edge coming from some segment to the depot vertex is just the time of travel between them, since depot vertex does not represent edge traversal.

The goal to be minimized, which for one agent multi-tour scenario is the min-sum of all tour costs, is:
\begin{equation}
   \min \sum_{m\in M}c(m) = \sum_{m\in M}\sum_{e \in m}c(e),
\end{equation}
constrained to maximum tour cost (maximum flight time or budget \Tmax):
\begin{equation}
   \sum_{e \in m}c(e) \leq \Tmax, \forall m \in M.
\end{equation}

, which is the main real-world constraint in the problem formulation.
\todo{formally define the travel cost of segment inspection and overflights between the pylons/segment end points}
%It is verified in~\ref{sec:results} that multi-rotor UAV is able to track these trajectories.

%Thus, the tour $T_i$ is a sequence of vertices $T_i=\{V_0, V^i_1,\ldots, V_1\}$ and for any tours $T_i,T_j\in\mathcal{T}$, it holds $T_i\bigcap T_j=\{V_0, V_1\}$.
\todo{notation of the vertices for the first and second directions of the segment inspection}
\todo{It might be more suitable to use $v_1$ instead of $V_1$.} 

%It is requested to start and terminate each inspection tour at the defined locations, and therefore $v_0 \in V$ and $v_1 \in V$ represent the corresponding starting and termination depot, respectively.


% - ilp.tex -------------------------------------------------------------------
Optimal solution can be obtained using integer linear programming.
In this section, it is assumed that $n = n_{vertex}$.
$C_{(n,n)}$ as a 2-dimensional asymmetric matrix of edge costs $c(e_{i,j})$ which are pre-computed,
$X_{(n_{tour},n,n)}$ as a 3-dimensional variable matrix, where elements $x_{m,i,j}$ denote traversal of these edges from $i$ to $j$ by a tour $m$.
It therefore specifies which edges are used by the tour, and the indexes $i,j \in E$ are relevant to previously defined set of edges $E$.
$T_{(n_{tour},n)}$ as 2-dimensional traversal matrix, where elements $t_{m,i}\in T$ denote the position of vertex $i$ in tour $m$. It specifies in which order the edges are used by the tour.
Since one vertex cannot repeat itself in a tour in this formulation, the depot vertices are represented as $v_0$ in outgoing case and $v_1$ in incoming case. Number of vertices is always even. The objective to be minimized is then:
The objective to be minimized is then:

It has to be ensured, that each pair of vertices belonging to a set (representing a line segment) is entered and exited exactly once. 
If a vertex is entered by a tour, it also has to be exited by the same tour:
\begin{equation}
   \sum_{i = 2}^{n/2}\sum_{j=0}^{n} x_{m,i,j} + x_{m,2i+1,j} = 1, \forall m \in M 
\end{equation}
\begin{equation}
   \sum_{i = 1}^{n/2} \sum_{j=0}^{n} x_{m,j,i} + x_{m,j,2i+1} = 1, \forall m\in M,
\end{equation}
\begin{equation}
   \sum_{i=2}^{n} x_{m,i,j} - x_{m,j,i} = 0, \forall m \in M, \forall 0 \leq j \le n,
\end{equation}
and the total cost of each tour is constrained. Here, $X_m$ denotes the square sub-matrix of $X$ containing variables for tour $m$:
\begin{equation}
   \sum_{(i,j)\in X_m}c_{m,i,j}x_{m,i,j} \leq \Tmax, \forall m \in M.
\end{equation}
Sub-tour elimination constraint (Miller-Tucker-Zemlin~\cite{miller60ilptsp}) is also included for each tour using matrix $T$:
\begin{equation}
   t_{m,i} - t_{m,j} + x_{m,i,j} \leq n - 1,  2 \leq i \neq j \leq n, \forall m \in M.
\end{equation}
This formulation can be used to solve the problem using off-the-shelf ILP solvers.
Cplex~\cite{cplex2009v12} solver is used to obtain our baseline solution.

\disable{
   \reviewiiiNote, the presented ILP formulation does not directly solve Problem~\ref{problem:mt-set-tsp} as the number of tours $n_t$ needs to be specified. 
   %The presented ILP formulation does not directly solve Problem~\ref{problem:mt-set-tsp} as the number of tours $n_t$ needs to be specified. 
   The minimal number of tours can be estimated by the solution of the TSP corresponding to a single-vehicle without the budget, e.g., using~\cite{concorde}.
   Then, the lower bound on the minimal number of the tours can be estimated by dividing the TSP solution cost by \Tmax{}. 
   Since such a number might be unrealistically low, the increased value can be utilized.
   In our case, the CPLEX solver determines feasibility of solution before solving, so the $n_s$ is iterated from the lowest value.
}

% - grasp.tex -----------------------------------------------------------------
Positions of all segments from the segment set $S_{initial}$ are directly manipulated in tours. 
The objective function is the sum of costs of all tours. 
Cost of a tour is time of travel from depot coordinates to the entry coordinate of first segment, then time of traversing the segment itself, then cost of traversing from exit coordinate to the entry coordinate of the next segment, and so on, until the last segment of tour is traversed when the return cost do the depot is added. 
If the soft constraint is violated, ie. if the tour cost $c(m)$ exceeds maximum allowed cost \Tmax, then the value of $k_{c}(c(m)-\Tmax)$ is added to the tour cost. 
Value $k_{c} = 1000$ represents a constraint constant by which the violation is multiplied. 
The only requirement is that the constant be a ``big enough'' number, so that the algorithm prioritizes reaching feasible solution.
As with the ILP formulation, costs of graph edges $c(e) \forall e \in E$ is pre-computed using a trajectory planner.
Time of pre-computation is negligible compared to the time spent solving, and provides a major speed-up to the algorithm.

In our case, $d$ is a boolean variable indicating if the set is traversed from first (to second coordinate or vice-versa. 
$I_{RCL}$ is a \emph{Restricted Candidate List} (RCL) of best insertion candidates, used randomize the GRP. 
In our case, the stopping criterion is no improvement of $S_{best}$ in 50 iterations.


In our case, $d$ is a Boolean variable indicating inspection direction; however, it can be an integer value in the case of further generalization.

% - results.tex ---------------------------------------------------------------
Several limits on flight time \Tmax were also chosen for each instance.
Computing cluster p
For computations, cloud computing cluster provided by project e-InfrastrukturaCZ was used. 
100 GB of RAM was allocated to each Cplex instance.

Both formulations and solvers were implemented in C++. 
is if the solution does not improve in 20 iterations. 

%\todo{add the supporting claims if possible}
%If GRASP failed to find a feasible solution, or Cplex ran out of memory,  the result is omitted.
%Cplex has a limit of about one day of computational time, which it reaches for larger problem instances shown in Table~\ref{table_comparison}.

For the GRASP procedure, values of several parameters are specified. 
As mentioned before, during the greedy random procedure, 

ILP formulaton and the Cplex solver are used to acquire optimal solution for each problem instance. 

Computational time of Cplex can also spike unpredictably depending on the mixture of constraints or quality of initial solution. It generally tends to increase exponentially with tighter \Tmax constraint and lower number of tours, as shown in~\ref{fig:d700}.

Optimal cost for each combination of constraints \Dmax and \Tmax is in bold, combinations are separated by horizontal lines.

GRASP solver took about \SI{1}{min} of CPU time on average for the largest instance \ref{fig:sol_big}. 

generally required to acquire best possible solution.

%and the percentage deviation between optimum solution cost provided by Cplex and best solution cost out of 30 provided by GRASP (referred to as PDB in~\ref{table_comparison}) is under $11\%$ for each problem instance. 

%\todo{define PDM or PDM and describe columns in the large table}
%Initializing Cplex from an existing solution provides significant performance improvement \textbf{table comparing them}.
%Since the computation cost of GRASP is very cheap, it does not make practical sense to solve the ILP without initialization.

%size of the problem, 
%In the performed empirically


%2, 3, 5 and 10 times the value of $\Dmax{}$ to create problem instances. $t_n$ between 3 and 6 is used to find feasible solutions.

The travel budget \Tmax{} is set to 2, 3, 5 and 10 times the value of $\Dmax{}$ to create problem instances. $t_n$ between 3 and 6 is used to find feasible solutions.

Therefore, we measure quality of the solution for the increased number of tours $n_t$ using and also for the heuristic GRASP-based solutions as the percentage deviation of the solution cost to the optimal solution cost $\%\textrm{PDB}=({\mathcal{C}-\mathcal{C}^*})/{\mathcal{C}^*} \cdot 100\%$, where $\mathcal{C}^*$ is the optimal solution cost found by the ILP solver.

%Due to the stochastic nature of the GRASP, multiple runs on a single instance are reported to show meaningful results.
Percentage deviation of average solution value is also included as \%PDM.


%Feasibility of the proposed PTL inspection planning has been empirically validated on a real-world dataset of the PTLs originating from substation Nechranice, courtesy of ČEPS, a.s. (Czech power transmission infrastructure institution, member of AERIAL~CORE advisory board).\footnote{The dataset is available for download at \url{http://mrs.felk.cvut.cz/mstsp-ptl-ral}.}

%\footnote{The dataset is available for download~\cite{mrs-mstsp}.}

%is also the most demanding solution in most of the cases.

% - conclusion.tex ------------------------------------------------------------

A novel TSP generalization has been presented in this paper, describing multi-tour set TSP.
The proposed approach is suitable for planning of PTL inspection by an autonomous multi-rotor UAV. 

and both solvers 
The optimization was formulated as an ILP, and solved using the Cplex solver.
A GRASP-based solver was also introduced, and its performance evaluated in comparison to the optimum provided by Cplex in several instances of the optimization problem.
Given a set of existing PTLs, it has been shown that the proposed GRASP solver can obtain solutions in a timespan by orders of magnitude shorter than the Cplex solver.
The feasibility of planned inspection trajectories has been verified.
The presented GRASP can provide solutions on-site and in real-time, where and when the inspection plan might change, as required by PTL operators, end-users of the proposed approach.



==> src/remove_grasp_solution.tex <==
% - section -------------------------------------------------------------------
\section{Proposed Heuristic Solver}\label{sec:grasp}
A GRASP-based heuristics algorithm is proposed.
It might not, and except for simple problem instances, does not, reach an optimal solution. 
It however provides a good-enough solution in a limited time span with faster convergence. 
Our algorithm is based on an existing planner for multi-product multi-vehicle routing problem \cite{guemri16or}, which we further generalize for set-TSP. 
Two meta-heuristics are used by our planner, a Greedy Random search Procedure (GRP), which obtains an initial and not necessarily feasible solution, followed by an adaptive Tabu Search (TS) to explore neighbourhood solutions using a set of specific moves. 
A soft constraint is used to limit maximum tour cost during the search. 
It is not guaranteed that the best solution found will be feasible, with respect to the maximum tour cost, so multiple iterations and increasing tour number might be required to guarantee feasibility.

Positions of all segments from the segment set $S_{initial}$ are directly manipulated in tours by the algorithm. 
The objective function is the sum of costs of all tours. 
Cost of a tour is time of travel from depot coordinates to the entry coordinate of first segment, then time of traversing the segment itself, then cost of traversing from exit coordinate to the entry coordinate of the next segment, and so on, until the last segment of tour is traversed when the return cost do the depot is added.
The costs are pre-computed and retrieved from the cost-matrix, as in ILP formulation.
If the soft constraint is violated, ie. if the tour cost $c(m)$ exceeds maximum allowed cost $T_{max}$, then the value of $k_{c}(c(m)-T_{max})$ is added to the tour cost. 
Value $k_{c} = 1000$ represents a constraint constant by which the violation is multiplied. 
The only requirement is that the constant be a "big enough" number, that the algorithm prioritizes reaching feasible solution.

\subsection{Greedy search procedure}
First, the initial solution is obtained using GRP, where $S_{initial}$ are all initial segments (or sets), $S_{available}$ is a list containing all unused segments, $I_{proposed}$ is a list of proposed insertions $i_{s,m,p,d}$ of some segment $s$, into tour $m$, at position $p$, in direction $d$, with known cost of solution after insertion Cost($i$).

In our case, $d$ is a simple boolean variable indicating if set is traversed from first to second coordinate or vice-versa. 
However, it can be an integer value for the purpose of set generalization. 
$I_{RCL}$ is Restricted Candidate Lists (RCL) of best insertion candidates, used randomize the GRP. 
The $I_{RCL}$ is chosen to contain $1/4$ of all the proposed insertions empirically, to get varied initial solutions.
\begin{algorithm}[htbp]
  \caption{Greedy Random Procedure $S_{initial}$}
    \label{alg:gr}
    \begin{algorithmic}[1] % The number tells where the line numbering should start
      \State $S_{available} \gets S_{initial}$
      \While{ size($S_{available}$) $\neq 0$}
        \State Fill $I_{proposed}$ with all possible insertions;
        \State Order elements of $I_{proposed}$ by Cost($i$);
        \State Fill $I_{RCL}$ with subset of $I_{proposed}$;
      \State $i_{selected} \gets$ Random $i$ from $I_{RCL}$;
      \State Insert $i_{selected}$ into route $m$;
      \State Remove $i_{selected}$, and other insertions referring to same segment set from $S_{available}$;
    \EndWhile
    \end{algorithmic}
\end{algorithm}
\subsection{Adaptive tabu search}
After initial greedy solution is obtained, adaptive tabu search is applied over several iterations to the routes. 
The solution space is explored by selecting from four distinct moves repeatedly, by weighted roulette wheel, as presented in \cite{guemri16or}. 
Similar moves are used to specify solution neighborhood, and one move for direction-switching is added, which hastens convergence to lower solution cost.
\begin{itemize}
\item Move 1 - 
\textit{Random-shift}: Remove a random segment from random route and insert it into random position in the same or other route. This move adds randomity to the search, and its score is increased every iteration.
\item Move 2 - 
\textit{Best-shift}: Remove a random segment from route and insert it into best position in the same or other route. Best insertion is found by exhaustive search from all possible insertions. 
\item Move 3 - 
\textit{Best-swap}: Swap a random segment from random route with the best segment in the same or other route. Best swap is, like in previous move, found by exhaustive search from all swaps.
\item Move 4 - 
\textit{Best-direction-switch}: Switch a traversal direction for best segment. Also evaluated over all segments.
\end{itemize}
The original position is never the same as destination position, ie. there is always some exploration of solution neigbourhood.
All possible moved segment directions are evaluated for first three moves, and the best one is chosen.

The score weight of each move ($w_i$ where $i \in 1 \ldots 4$) is initialized at $w_0$, and is increased every iteration according to performace. 
Two prize values are used, $p1$ and $p2$. 
$p1$ is added to the best move in the neighbourhood, $p2$ is added to the move which improved best overall TS solution. 
Value of $p1$ is added to to the weight $w_1$ every iteration, to promote randomness in neigbourhood exploration and to escape local optima. 
Every $R_t$ iterations, the score weights are reinitialized at $w_0$. Neighbourhood of size $n^2$ is explored, using tabu list $T_{list}$ of $T_{size}$. 

The tabu search algorithm is outlined in pseudo-code. 
Here, $S$ denotes some existing solution, $T_{list}$ a tabu list of explored solutions and $N(S)$ a neighbourhood of some solution $S$. 
In our case, the stopping criterion is no improvement of $S_{best}$ in 50 iterations.
\begin{algorithm}[htbp]
  \caption{Tabu Search ($S$)}
    \label{alg:tabu}
    \begin{algorithmic}[1] % The number tells where the line numbering should start
      \State $S_{best} \gets S$
      \State $S_{current} \gets S$
      \State Insert $S_{current}$ into $T_{list}$
      \While{Stopping criterion not met}
       \State Create solution neighborbood $N(S_{current})$
       \State $S_{current} \gets $Best\{$S \in N(S_{current})$ and $S \notin T_{list}$\}
       \If{Cost($S_{current}$) $<$ Cost($S_{best}$)}
       \State $S_{best} \gets S_{current}$
       \EndIf
      \EndWhile
      \State \Return $S_{best}$
    \end{algorithmic}
\end{algorithm}


==> tbl/result_data.tex <==
{500}&{1000}&{4}&{7.4}&\textbf{3178.75}&{0.0}&&{0.05}&{1.639}&{3506.5}&{10.3}&{3499.67}&{10.1}\\ 
{500}&{1000}&{5}&{2.6}&3221.43&{1.3}&&{0.08}&{2.269}&{3397.4}&{6.9}&{3370.99}&{6.0}\\ 
{500}&{1000}&{6}&{0.9}&3328.4&{4.7}&&{0.04}&{1.344}&{3566.6}&{12.2}&{3478.38}&{9.4}\\ 
\hline 
{500}&{1500}&{3}&{1.9}&\textbf{3053.15}&{0.0}&&{0.06}&{1.764}&{3281.7}&{7.5}&{3262.43}&{6.9}\\ 
{500}&{1500}&{4}&{1.4}&3087.88&{1.1}&&{0.12}&{3.466}&{3321.7}&{8.8}&{3260.08}&{6.8}\\ 
{500}&{1500}&{5}&{1.2}&3194.85&{4.6}&&{0.05}&{1.49}&{3458.4}&{13.3}&{3448.09}&{12.9}\\ 
{500}&{1500}&{6}&{0.8}&3296.05&{8.0}&&{0.05}&{1.576}&{3492.2}&{14.4}&{3452.7}&{13.1}\\ 
\hline 
{600}&{1800}&{3}&{74.1}&\textbf{5143.38}&{0.0}&&{0.07}&{2.146}&{5582.9}&{8.5}&{5497.46}&{6.8}\\ 
{600}&{1800}&{4}&{46.3}&5176.84&{0.7}&&{0.15}&{4.632}&{5645.5}&{9.8}&{5590.65}&{8.7}\\ 
{600}&{1800}&{5}&{35.5}&5244.62&{2.0}&&{0.11}&{3.247}&{5764.9}&{12.1}&{5705.24}&{10.9}\\ 
{600}&{1800}&{6}&{39.4}&5356.32&{4.1}&&{0.13}&{4.006}&{5843.6}&{13.6}&{5701.55}&{10.9}\\ 
\hline 
{600}&{3000}&{3}&{12.1}&\textbf{5090.41}&{0.0}&&{0.18}&{5.363}&{5562.5}&{9.3}&{5460.44}&{7.3}\\ 
{600}&{3000}&{4}&{11.9}&5161.97&{1.4}&&{0.08}&{2.49}&{5595.4}&{9.9}&{5464.18}&{7.3}\\ 
{600}&{3000}&{5}&{10.9}&5229.75&{2.7}&&{0.13}&{3.778}&{5698.6}&{11.9}&{5661.88}&{11.2}\\ 
{600}&{3000}&{6}&{12.9}&5344.06&{5.0}&&{0.16}&{4.838}&{5878.6}&{15.5}&{5796.44}&{13.9}\\ 
\hline 
{700}&{2100}&{4}&{51355.1}&\textbf{6268.27}&{0.0}&&{0.17}&{5.211}&{6951.6}&{10.9}&{6736.48}&{7.5}\\ 
{700}&{2100}&{5}&{3838.8}&6321.05&{0.8}&&{0.14}&{4.077}&{6986.3}&{11.5}&{6717.39}&{7.2}\\ 
{700}&{2100}&{6}&{194.3}&6416.85&{2.4}&&{0.2}&{6.127}&{7042.3}&{12.3}&{6928.91}&{10.5}\\ 
\hline 
{700}&{3500}&{3}&{6401.6}&\textbf{6161.78}&{0.0}&&{0.29}&{8.609}&{6700.0}&{8.7}&{6526.08}&{5.9}\\ 
{700}&{3500}&{4}&{2755.7}&6222.44&{1.0}&&{0.19}&{5.708}&{6748.6}&{9.5}&{6637.07}&{7.7}\\ 
{700}&{3500}&{5}&{328.7}&6289.68&{2.1}&&{0.43}&{12.882}&{6880.6}&{11.7}&{6716.01}&{9.0}\\ 
{700}&{3500}&{6}&{188.4}&6415.72&{4.1}&&{0.2}&{6.007}&{7118.6}&{15.5}&{7024.6}&{14.0}\\ 
\hline 
{700}&{7000}&{3}&{1166.0}&\textbf{6143.87}&{0.0}&&{0.22}&{6.495}&{6738.6}&{9.7}&{6514.55}&{6.0}\\ 
{700}&{7000}&{4}&{290.0}&6211.1&{1.1}&&{0.17}&{5.136}&{6770.8}&{10.2}&{6654.99}&{8.3}\\ 
{700}&{7000}&{5}&{316.4}&6289.68&{2.4}&&{0.44}&{13.28}&{6965.3}&{13.4}&{6769.32}&{10.2}\\ 
{700}&{7000}&{6}&{122.1}&6415.72&{4.4}&&{0.22}&{6.611}&{7034.6}&{14.5}&{6933.07}&{12.8}\\ 
\hline 
{800}&{2400}&{5}&{15765.0}&\textbf{7509.96}&{0.0}&&{0.19}&{5.77}&{8420.8}&{12.1}&{8234.65}&{9.6}\\ 
{800}&{2400}&{6}&{2807.3}&7602.37&{1.2}&&{0.28}&{8.542}&{8421.3}&{12.1}&{8288.05}&{10.4}\\ 
\hline 
{800}&{4000}&{3}&{24120.2}&\textbf{7369.24}&{0.0}&&{0.39}&{11.636}&{8058.1}&{9.3}&{7879.37}&{6.9}\\ 
{800}&{4000}&{4}&{769.0}&7403.97&{0.5}&&{0.35}&{10.559}&{8210.2}&{11.4}&{8020.51}&{8.8}\\ 
{800}&{4000}&{5}&{24379.7}&7487.94&{1.6}&&{0.46}&{13.907}&{8285.1}&{12.4}&{8081.83}&{9.7}\\ 
{800}&{4000}&{6}&{1770.0}&7602.37&{3.2}&&{0.49}&{14.73}&{8482.1}&{15.1}&{8289.55}&{12.5}\\ 
\hline 
{800}&{8000}&{3}&{1003.0}&\textbf{7318.65}&{0.0}&&{0.44}&{13.28}&{8104.1}&{10.7}&{7938.3}&{8.5}\\ 
{800}&{8000}&{4}&{1054.9}&7403.97&{1.2}&&{0.35}&{10.393}&{8244.4}&{12.6}&{7854.32}&{7.3}\\ 
{800}&{8000}&{5}&{5203.3}&7487.94&{2.3}&&{0.32}&{9.708}&{8345.9}&{14.0}&{8115.01}&{10.9}\\ 
{800}&{8000}&{6}&{2755.2}&7602.37&{3.9}&&{0.25}&{7.429}&{8525.5}&{16.5}&{8419.58}&{15.0}\\ 
\hline 
{900}&{2700}&{6}&{10661.1}&\textbf{9014.37}&{0.0}&&{0.59}&{17.761}&{10210.4}&{13.3}&{9933.18}&{10.2}\\ 
\hline 
{900}&{4500}&{3}&{35372.2}&\textbf{8782.42}&{0.0}&&{0.64}&{19.054}&{9804.2}&{11.6}&{9600.31}&{9.3}\\ 
{900}&{4500}&{4}&{1004.2}&8817.14&{0.4}&&{0.53}&{15.867}&{9906.9}&{12.8}&{9631.81}&{9.7}\\ 
{900}&{4500}&{5}&{26029.7}&8884.38&{1.2}&&{0.87}&{25.973}&{10108.4}&{15.1}&{9808.96}&{11.7}\\ 
{900}&{4500}&{6}&{3506.5}&9006.59&{2.6}&&{0.52}&{15.465}&{10246.7}&{16.7}&{9985.96}&{13.7}\\ 
\hline 
{900}&{9000}&{3}&{1492.3}&\textbf{8738.75}&{0.0}&&{0.54}&{16.328}&{9780.9}&{11.9}&{9399.0}&{7.6}\\ 
{900}&{9000}&{4}&{8954.6}&8814.28&{0.9}&&{0.63}&{18.936}&{9920.5}&{13.5}&{9740.36}&{11.5}\\ 
{900}&{9000}&{5}&{721.4}&8884.38&{1.7}&&{0.49}&{14.678}&{10083.3}&{15.4}&{9744.84}&{11.5}\\ 
{900}&{9000}&{6}&{3251.9}&9006.59&{3.1}&&{0.56}&{16.754}&{10244.6}&{17.2}&{9980.26}&{14.2}\\ 
\hline 
{1000}&{3000}&{6}&{21174.5}&\textbf{9887.62}&{0.0}&&{0.65}&{19.505}&{11130.4}&{12.6}&{10869.6}&{9.9}\\ 
\hline 
{1000}&{5000}&{4}&{86370.0}&\textbf{9712.65}&{0.0}&&{0.62}&{18.476}&{10845.0}&{11.7}&{10544.2}&{8.6}\\ 
{1000}&{5000}&{6}&{13605.2}&9887.62&{1.8}&&{0.63}&{18.972}&{11112.0}&{14.4}&{10917.7}&{12.4}\\ 
\hline 
{1000}&{10000}&{3}&{51951.8}&\textbf{9616.89}&{0.0}&&{0.73}&{21.768}&{10627.5}&{10.5}&{10318.8}&{7.3}\\ 
{1000}&{10000}&{4}&{86370.0}&9708.18&{0.9}&&{0.59}&{17.789}&{10819.3}&{12.5}&{10521.7}&{9.4}\\ 
{1000}&{10000}&{5}&{86370.0}&9779.16&{1.7}&&{0.46}&{13.688}&{11021.6}&{14.6}&{10678.0}&{11.0}\\ 
{1000}&{10000}&{6}&{48811.4}&9887.62&{2.8}&&{0.63}&{18.887}&{11212.8}&{16.6}&{10876.5}&{13.1}\\ 
\hline 
{1100}&{5500}&{4}&{86370.1}&\textbf{11113.4}&{0.0}&&{1.5}&{45.142}&{12407.4}&{11.6}&{12144.0}&{9.3}\\ 
\hline 
{1100}&{11000}&{3}&{59362.5}&\textbf{10995.0}&{0.0}&&{1.11}&{33.375}&{12196.8}&{10.9}&{11988.4}&{9.0}\\ 
{1100}&{11000}&{4}&{86370.0}&11078.4&{0.8}&&{0.68}&{20.273}&{12372.6}&{12.5}&{12168.8}&{10.7}\\ 
{1100}&{11000}&{5}&{9371.1}&11179.8&{1.7}&&{0.77}&{23.208}&{12565.2}&{14.3}&{12233.3}&{11.3}\\ 
\hline 
{1200}&{12000}&{4}&{86370.1}&\textbf{12453.0}&{0.0}&&{0.76}&{22.796}&{13870.3}&{11.4}&{13567.6}&{9.0}\\ 
{1200}&{12000}&{5}&{86370.0}&12564.0&{0.9}&&{1.03}&{30.827}&{14044.0}&{12.8}&{13502.2}&{8.4}\\ 
\hline 
{1300}&{6500}&{3}&{86370.1}&\textbf{13184.1}&{0.0}&&{1.66}&{49.722}&{14462.8}&{9.7}&{14160.5}&{7.4}\\ 
\hline 
{1300}&{13000}&{3}&{86370.0}&\textbf{13143.8}&{0.0}&&{1.31}&{39.327}&{14476.4}&{10.1}&{14156.6}&{7.7}\\ 
\hline 
{1500}&{15000}&{4}&{86370.1}&\textbf{15860.6}&{0.0}&&{1.75}&{9.806}&{17637.8}&{11.2}&{17258.8}&{8.81}\\ 


==> tbl/result_table.tex <==

    \begin{table*}[h]
        \caption{Comparison of solutions}
        \label{tbl:table_comparison}
        \begin{center}
          \resizebox{\textwidth}{!}{
            \begin{tabular}{
            c
            c
            c
            r
            r
            r
            r
            r
            r
            r
            r
            r
            r
            }
                \hline
                \multicolumn{3}{c}{} &\multicolumn{3}{c}{Cplex ILP} && \multicolumn{6}{c}{GRASP} \\
                \cline{4-6}\cline{8-13}
                \Dmax [\si{m}] & \Cmax [\si{s}] & $n_{t}$ & t [\si{s}] & $\mathcal{C}^*$ [\si{s}] & PDB [\%] && t\textsubscript{avg} [\si{s}] & t\textsubscript{sum} [\si{s}] & $\mathcal{C}_{avg}$ [\si{s}] & PDA [\%]& $\mathcal{C}_{best}$ [\si{s}]& PDB [\%] \\
                \hline
\input{tbl/result_data.tex}
\hline
            \end{tabular}}
        \end{center}
    \end{table*}

